What comes next? Extractive summarization by next-sentence prediction

Existing approaches to automatic summarization assume that a length limit for the summary is given, and view content selection as an optimization problem to maximize informativeness and minimize redundancy within this budget. This framework ignores the fact that human-written summaries have rich internal structure which can be exploited to train a summarization system. We present NEXTSUM, a novel approach to summarization based on a model that predicts the next sentence to include in the summary using not only the source article, but also the summary produced so far. We show that such a model successfully captures summary-specific discourse moves, and leads to better content selection performance, in addition to automatically predicting how long the target summary should be. We perform experiments on the New York Times Annotated Corpus of summaries, where NEXTSUM outperforms lead and content-model summarization baselines by significant margins. We also show that the lengths of summaries produced by our system correlates with the lengths of the human-written gold standards.

==> abstract.tex <==
  %Summarization systems are becoming rather good at selecting important content for
  %summaries. The selection of sentences however is done either independently or using
  %global optimization procedure such as Integer Linear Programming. In this work, we
  %present a new way of approaching the sentence selection problem such that summaries
  %are locally tight with respect to topic and content. 
  %Central to our work is a next sentence prediction model which selects the
  %next summary sentence given the sentences in the summary so far.
  %We show that such a model can capture summary specific discourse moves
  %and leads to better sentence selection performance in a summarization system.
  %We perform experiments on the New York
  %Times Annotated Corpus of summaries, where our system outperforms lead and
  %content summarization baselines with a significant margin. 
  

Existing approaches to automatic summarization assume a given summary 
length limit, and view content selection as an optimization problem to 
maximize informativeness and minimize redundancy within this budget. This 
setup ignores the fact that human-written summaries have rich internal 
structure which can be exploited to train a summarization system. In 
this work, we present \textsc{NextSum}, a novel approach to 
summarization based on a module that predicts the next summary sentence
using not only the source article, but also 
the sentences in the summary so far. We show that such a model 
successfully captures summary-specific discourse moves, and leads
to better content selection performance, in addition to automatically
predicting how long the target summary should be. We perform experiments on the New York Times 
Annotated Corpus of summaries, where \textsc{NextSum} outperforms lead and content-model 
summarization baselines by significant margins. We also show that the lengths of 
summaries produced by our system correlates with the lengths of the 
human-written gold standards.
	


==> intro.tex <==
\section{Introduction}

Writing a summary is a different task compared to producing a longer
article. As a consequence, it is likely that the topic and 
discourse \emph{moves} made in summaries differ from those in regular 
articles. In this work, we present a powerful extractive summarization system 
which exploits rich summary-internal structure to 
perform content selection, redundancy reduction, and even predict
the target summary length, all in one joint model. 

% Text summarization is an important application which has been addressed by 
% numerous techniques in the community \cite{nenkova-mckeown:2011}. In this
% work, we present a new approach to extractive summarization. 
% Our core idea is based on the intuition that summary writing may involve 
% predictable discourse and topic moves and these can be learned from 
% large collections of summaries. Summarization systems can become 
% more powerful by learning to exploit this rich 
% summary-internal structure.
% % The key idea we propose is that since summaries in a domain often follow some 
% % predictable structure, a partial summary or set of summary sentences should help 
% % predict other summary sentences. 
% We formalize this intuition in a model 
% called \textsc{NextSum}, which builds summaries incrementally by observing 
% properties of not just the source but also the previously selected sentences
% in the summary so far. 
% % which selects the next summary sentence based not only on 
% % properties of the source text, but also on the previously selected sentences in the summary. 

Text summarization has been addressed by 
numerous techniques in the community \cite{nenkova-mckeown:2011}.
For extractive summarization, which is the focus of this paper, a popular task setup is
to generate summaries that respect a fixed length limit. For 
example, summarization shared tasks in the past Document 
Understanding Conferences (DUC\footnote{\url{http://duc.nist.gov/}}) 
define these limits in terms of words or bytes. As a result, 
much work has framed summarization
as a constrained optimization problem, in 
order to select a subset of sentences that achieve desirable summary qualities 
such as informativeness, coherence, and 
non-redundancy within the length budget.
\cite{gillick-favre:2009,lin-bilmes:2011,kulesza-taskar:2011}. 

One problem with this setup is that it
does not match many real-world summarization settings. 
For example, writers can tailor the length of 
their summaries to the amount of noteworthy content 
in the source article. Summaries created by news editors for archives 
on the New York Times Annotated Corpus \cite{NYTcorpus} exhibit a variety of lengths. 
There is also evidence that in the context of web search, people prefer summaries 
of different lengths for the documents in search results depending on the type 
of search query \cite{kaisser-hearst-lowe:2008}. More generally, current systems
focus heavily on identifying which properties of the source document can 
point to important sentences and help score the coherence of transitions 
between them. They reason about summary content primarily for 
purposes of avoiding redundancy and respecting the length budget. 
But they ignore the idea that it might actually be useful
to learn content structure and discourse planning for summaries from large 
collections of multi-sentence summaries. 

This work proposes an extractive summarization system that focuses on 
capturing rich summary-internal structure. Our key idea is that 
since summaries in a domain often follow some 
predictable structure, a partial summary or set of summary sentences should help 
predict other summary sentences. 
We formalize this intuition in a model 
called \textsc{NextSum}, which selects the next summary sentence based not only on 
properties of the source text, but also on the previously 
selected sentences in the summary. 
This setup allows our model to capture \emph{summary-specific discourse and topic transitions}. 
For example, it can learn to expand on a topic that is already 
mentioned in the summary, or to introduce a new topic. It can 
learn to follow a script or discourse relations that are 
expected for that domain. It can even learn to predict the end of the summary, avoiding 
the need to explicitly define a length cutoff. 


% there is rich and 
% useful internal structure within multi-sentence 
% human-written summaries which are little explored in 
% current summarization systems. For example, given an article about a celebrity
% divorce, one can predict that a summary will contain 
%%AL appears too similar to content models, so commenting for now. And also 
%%we need to distinguish the topic structure of source from summaries.
% For example, a summary about a 
% celebrity divorce might begin by stating who the celebrities are, then discuss 
% the cause of the break-up, followed by child custody arrangements. In addition to
% topic structure, summaries may make different discourse moves compared to long
% articles. 
% Our work differs from previous approaches that reason about summary-internal structure, 
% which do so primarily for the purposes of avoiding redundancy \cite{nallapat-etal:2017}, 
% or improving local discourse coherence \cite{christensen-etal:2013}.

The core of our system is a next-sentence prediction component, which is a 
feed-forward neural network driven by features capturing the prevalence of 
domain subtopics in the source and the summary, sentence importance in the source, and 
coverage of the source document by the summary so far. % A parallel to this work 
% can be found in recent work in dialogue systems, in which systems are trained to predict 
% the next dialogue utterance from among a set of candidates \cite{lowe-etal:2016}. 
A full summary can then be generated by repeatedly predicting the next sentence until 
the end of a summary is predicted.
(TODO: An example of the setup of our approach is shown in Figure~\ref{}.)
\thoughts{Need an example from our dataset; two sample next sentences; both are good 
candidates in the summary overall, but clearly only one should be selected.}

Since the use of summary-specific moves may depend on the specific domain 
being summarized, we first explore domain-specific summarization systems on 
event-oriented news topics (War Crimes, Assassinations, Bombs) from the
 New York Times Annotated Corpus \cite{NYTcorpus}. We then show that the model is 
also powerful in a domain-general setting across 
multiple types of events.
Within \textsc{NextSum}, next summary sentence prediction can be done with 
remarkably high accuracies, reaching 67\% compared to a chance-level performance of 9\%. 
The generated summaries outperform the lead baseline 
as well as several domain-specific summarization baselines without requiring explicit 
redundancy check or a length constraint. Moreover, summary termination works 
well within the same model, and we show that the system produces summaries of 
variable lengths which correlate with how long human summaries are for the same texts. 



==> relwk.tex <==
\section{Related work}

%Many extractive summarization systems are unsupervised. The sentence scores
%were obtained through functions on word frequency \cite{} or computed on a graph representation of 
%the input sentences \cite{}. The summary is created by including the highest 
%scoring sentences, either greedily or using a global optimization procedure 
%such as ILP \cite{}. Non-redundancy and length limit act as constraints during 
%selection. 

Many previous approaches to extractive summarization have been unsupervised, and 
focus on the role of word frequency and source document representation
for selecting informative and non-redundant content \cite{Drago04,Rada04,nenkova06}.
More recently, supervised approaches have been proposed, which view content 
selection as a sentence-level binary classification problem, typically 
using a neural network \cite{cheng-lapata:2016,Nallapati2017}.

\paragraph{Using source structure.} % Many summarization
% techniques focus on computing the salience of words and sentences in the source by 
% looking at the frequency of words or relative position of sentences 
% within the source.
% Explicit relationships
% between source words or sentences are also computed in graph 
% based summarization techniques. The edges
% are based on similarity in content of words and sentences, and an algorithm such as PageRank then
% scores the nodes for importance.
Source structure is a common cue for summarization and can be explicitly 
observed in discourse- and graph-based summarization techniques 
\cite{marcu98,louis-joshi-nenkova:2010:SIGDIAL,christensen-etal:2013}. 
%For example,  in G-FLOW \cite{}, a graph is created
%for every source document where edges reflect how much one sentence is likely to flow
%from another defined by discourse, temporal and other coherence
%factors in the source. A candidate summary in G-FLOW is a 
%sequence of sentences, and is scored by how much the sequence
%preserves the coherence relations of this source graph. 
There are also techniques which learn probabilistic topic models over the source
domain in order to capture subtopics and transitions between them from hundreds of 
documents taken from the same domain \cite{haghighi2009,P13-1039}. 
The use of structure from summaries is less explored. 

\paragraph{Using summary structure.} 
In fact, almost all systems maintain some representation of the partial summary at a timestep. 
At the very least, it is needed for respecting a length limit and for preventing redundancy.
For example, the recent model of \newcite{Nallapati2017}, maintains a representation of the
summary so far and uses it to reduce redundancy in sentence selection. 
However, current methods do not focus on capturing rich summary discourse and 
content structure, which is the focus of our work. 

%The currently popular neural network based extractive systems
%predict the summary-worthiness of sentences based on the sentence and document representation, but each
%sentence is individually scored for summary worthiness and the top sentences are selected up to the 
%desired summary length.

Recent abstractive neural summarization models based on encoder-decoder 
frameworks actually have greater scope for capturing summary structure 
and content. The use of techniques such as attention and pointer mechanisms 
can be viewed as a form of summary structure 
modelling \cite{rush-chopra-weston:2015,see-liu-manning:2017}.
However, because such systems currently operate at the word level, 
these mechanisms are mostly used for 
handling issues such as grammaticality, out-of-vocabulary items, 
predicate-argument structure, and local coherence. 
By contrast, we aim to capture higher-level transitions in the contents of a summary.

%In fact, abstractive summarization in the recent neural network 
%approach are an exception, and do have scope for capturing summary structure and content. 
%These systems are mostly 
%based on sequence-to-sequence learning in an encoder-decoder framework. The decoder is a recurrent
%neural network which generates one word at a time conditioned on the 
%previously generated words as well as the source representation. 
%But these systems are currently small-scale, generating short headlines 
%from a sentence or two \cite{}. At other times, they generate story highlights 
%which are often disconnected sentences and do not make up a coherent 
%story \cite{}. (Need to talk about Pointer net paper and Socher)
%Our work is the first to explicitly train a 
%model to predict the next content in a partial summary. 

\paragraph{Next-sentence prediction.} The core of our system is a module to perform next summary sentence 
prediction. A parallel idea can be found in the form of  next-utterance prediction in 
retrieval-based dialogue systems \cite{lowe-etal:2016}. 
There have also been recent attempts at predicting the
next sentence in text. The skip-thought model \cite{Kiros2015} is trained to 
predict a sentence from its neighbouring
sentences in order to produce better sentence representations. 
\newcite{CLSTM2016} test a neural language model on 
the task of next-sentence prediction, and \newcite{pichotta:acl16} 
evaluate next sentence prediction as a proxy for 
predicting the next events in a discourse.  Our work 
differs in that it aims to predict the next output sentence
within the tangible application of summarization.

%\paragraph{Constraints during content selection.} There are typically two constraints, the summary length
%and non-redundancy. The length of a summary is typically input to summarization
%systems (e.g., 100 or 200 words in several DUC or TAC shared tasks). 
%In large corpora of summaries, it is rather common to have summaries of widely varying
%length. In systems that generate summaries for such corpora, the oracle length of each summary 
%is also input to the system \cite{}. Very little work has shown how one might predict the necessary
%compression given a source document. For non-redundancy, systems either perform an 
%explicit check to see if a new sentence is very similar to those already in the summary or 
%the similarity score between sentences is a negative score during global optimization in ILP. 
%In this work, we show how a next sentence prediction model can naturally incorporate both length and non-redundancy during summarization. 
% JC: We've already made this point, right? Removing for now.


